Regulator constants of integral representations of finite groups

Let G be a finite group and p be a prime. We investigate isomorphism invariants of $\mathbb{Z}_{p}[G]$-lattices whose extension of scalars to $\mathbb{Q}_p$ is self-dual, called regulator constants. These were originally introduced by Dokchitser--Dokchitser in the context of elliptic curves. Regulator constants canonically yield a pairing between the space of Brauer relations for G and the subspace of the representation ring for which regulator constants are defined. For all G, we show that this pairing is never identically zero. For formal reasons, this pairing will, in general, have non-trivial kernel. But, if G has cyclic Sylow p-subgroups and we restrict to considering permutation lattices, then we show that the pairing is non-degenerate modulo the formal kernel. Using this we can show that, for certain groups, including dihedral groups of order 2p for p odd, the isomorphism class of any $\mathbb{Z}_p[G]$-lattice whose extension of scalars to $\mathbb{Q}_p$ is self-dual, is determined by its regulator constants, its extension of scalars to $\mathbb{Q}_p$, and a cohomological invariant of Yakovlev.

==> functions.tex <==
\NeedsTeXFormat{LaTeX2e}
%\ProvidesPackage{functions}[Functions via a common preamble]

\newcommand{\z}{\mathbb{Z}} 
\newcommand{\n}{\mathbb{N}}
\newcommand{\co}{\mathbb{C}}
\newcommand{\q}{\mathbb{Q}}
\newcommand{\re}{\mathbb{R}}
\newcommand{\cha}{\text{char}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\A}{\mathbb{A}}
\newcommand{\CRng}{\text{CRng}}
\newcommand{\one}{\mathbbm{1}}
%\newcommand{\rk}{\operatorname{ rk}\hspace{1pt} }
\DeclareMathOperator{\rk}{rk}
\newcommand{\id}{\operatorname{ id}}
\newcommand{\tr}{\operatorname{ tr}}
%\newcommand{\ker}{\operatorname{ ker}}
\newcommand{\im}{\operatorname{ im}}
\newcommand{\cl}{\operatorname{ Cl}}
\newcommand{\obj}{\operatorname{ Obj}}
\newcommand{\proj}{\operatorname{ Proj}}
\newcommand{\Der}{\operatorname{ Der}}
\newcommand{\Set}{\operatorname{ Set}}
\newcommand{\res}{\operatorname{res}}
\newcommand{\Ind}{\operatorname{Ind}}
\newcommand{\Res}{\text{Res}}
\newcommand{\g}{\mathfrak{g}}
\newcommand{\kf}{\mathfrak{k}}
\newcommand{\Grp}{\text{Grp}}
\newcommand{\p}{\mathfrak{p}}
\newcommand{\C}{\mathscr{C}}
\newcommand{\ok}{\mathcal{O}_K}
\newcommand{\of}{\mathcal{O}_F}
\newcommand{\ol}{\mathcal{O}_L}
\newcommand{\OO}{\mathcal{O}}
\newcommand{\Nm}{\operatorname{ Nm}}
\newcommand{\SL}{\operatorname{ SL}}
\renewcommand{\sl}{ \mathfrak{sl}}
\newcommand{\GL}{\operatorname{ GL}}
\newcommand{\gl}{ \mathfrak{gl}}
\newcommand{\SO}{\operatorname{ SO}}
\newcommand{\SU}{\operatorname{ SU}}
\newcommand{\Gr}{\operatorname{ Gr}}
\newcommand{\Br}{\operatorname{ Br}}
\newcommand{\gal}{\operatorname{ Gal}}
\newcommand{\Aut}{\operatorname{ Aut}}
\newcommand{\Div}{\operatorname{ Div}}
\newcommand{\Pic}{\operatorname{ Pic}}
\newcommand{\Spec}{\operatorname{{ Spec}}}
\newcommand{\Spf}{\operatorname{Spf}}
\newcommand{\Hom}{\operatorname{ Hom}}
\newcommand{\Sel}{\operatorname{ Sel}}
\newcommand{\ind}{\operatorname{ ind}}
\newcommand{\ress}{\operatorname{ res}}
\newcommand{\cores}{\operatorname{ cores}}
\newcommand{\tors}{\text{tors}}
\newcommand{\coker}{\operatorname{ coker }\;}
\newcommand{\inv}{\operatorname{ inv}}
\newcommand{\fix}{\operatorname{ Fix}}
\newcommand{\hc}{H_{\! \! \text{ \rm cont}}^*}
\newcommand{\htop}{H_{\! \!\text{ \rm top}}^*}
\newcommand{\hgr}{H_{\! \text{ \rm grp}}^*}
\newcommand{\plgr}{P^{\! \text{ \rm grp}}_*}
\newcommand{\hlgr}{H^{\!\text{ \rm grp}}_*}
\newcommand{\hs}{H^*}
\newcommand{\Sch}{\operatorname{ Sch}}
\newcommand{\hls}{H_*}
\newcommand{\hcn}{H_{\! \! \text{ \rm cont}}}
\newcommand{\htopn}{H_{\! \!\text{ \rm top}}}
\newcommand{\hltopn}{H^{\!\text{ \rm top}}}
\newcommand{\hgrn}{H_{\! \!\text{ \rm grp}}}
\newcommand{\plgrn}{P^{\!\text{ \rm grp}}}
\newcommand{\hlgrn}{H^{\!\text{ \rm grp}}}
\newcommand{\lie}{\operatorname{ Lie}}
\newcommand{\st}{\;|\:}
\newcommand{\tss}{\textsuperscript}
\newcommand{\eps}{\epsilon}
\newcommand{\ti}{\times}
\newcommand{\Tr}{\operatorname{ Tr}}
\newcommand{\End}{\operatorname{ End}}
\renewcommand{\L}{\mathcal{L}}
\newcommand{\G}{\mathbb{G}}
\newcommand{\T}{\mathbb{T}}
\newcommand{\FF}{\mathscr{F}}
\newcommand{\Proj}{\text{Proj}}
\newcommand{\Map}{\text{Map}}
\newcommand{\Irr}{\text{Irr}}
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\qq}{\mathfrak{q}}
\newcommand{\s}{\mathfrak{s}}
\newcommand{\D}{\mathscr{D}}
\renewcommand{\AA}{\mathscr{A}}
\newcommand{\Frob}{\text{Frob}}
\newcommand{\Stab}{\text{Stab}}
\newcommand{\opp}{\text{op}}
\newcommand{\h}{\text{h}}
\newcommand{\sh}{\text{sh}}
\newcommand{\etale}{\'{e}tale }
%\newcommand{\et}{\'{e}t}
\newcommand{\unr}{{\rm unr}}
\newcommand{\tame}{{\rm tame}}
\newcommand{\ze}{\zeta}
\renewcommand{\a}{\mathfrak{a}}
\usepackage{letltxmacro}
\LetLtxMacro{\temp}{\phi}
\LetLtxMacro{\phi}{\varphi}
\LetLtxMacro{\varphi}{\temp}


% Text + Styles
\renewcommand{\th}{{\tss{th}} }
\renewcommand{\st}{{\ | \ }}
\newcommand{\ba}{\backslash}

% General Functions

%\DeclareMathOperator*{\sup}{sup}
%\DeclareMathOperator*{\inf}{inf}
\newcommand{\bac}{\backslash}
\newcommand{\pp}{\mathcal{P}}
\newcommand{\R}{\mathcal{R}}

%\newcommand{\End}{\operatorname{End}}
\newcommand{\ab}{\text{ab}}
%\newcommand{\ti}{\times}
\newcommand{\tii}{^\times}
\newcommand{\ot}{\otimes}
\newcommand{\op}{\oplus}
\newcommand{\ord}{\operatorname{ord}}

% Algebra

\newcommand{\PSL}{\operatorname{PSL}}

% Algebraic Number Theory
\newcommand{\Reg}{\operatorname{Reg}}
\newcommand{\cyc}{\text{{\rm cyc}}}
%\newcommand{\ab}{\text{ab}}
%\newcommand{\A}{\mathbb{A}}

% Commutative Algebra

\newcommand{\cor}{\operatorname{cor}}
\newcommand{\zp}{\z_{(p)}}

% Algebraic Geometry
\newcommand{\PP}{\mathbb{P}}
\newcommand{\dR}{\text{dR}}
\newcommand{\HT}{\text{HT}}
\newcommand{\cris}{\text{cris}}
\newcommand{\sta}{\text{st}}
\newcommand{\et}{\text{\'{e}t}}
\renewcommand{\div}{\operatorname{div}}
\newcommand{\Ell}{\text{Ell}}

%\newcommand{\FF}{\mathscr{F}}
\newcommand{\fppf}{\text{fppf}}
\newcommand{\fpqc}{\text{fpqc}}

% Representation Theory

\newcommand{\Lift}{\operatorname{Lift}}
\newcommand{\rti}{\rtimes}
\newcommand{\triv}{\text{{\rm triv}}}
\newcommand{\nt}{\text{{\rm nt}}}
\newcommand{\up}{\!\uparrow}
\newcommand{\down}{\!\downarrow}


% Modular Forms

\newcommand{\hh}{\mathcal{H}}
\newcommand{\M}{\mathcal{M}}
\renewcommand{\SS}{\mathcal{S}}
\newcommand{\Cusps}{\text{Cusps}}

% LaTeX

\newcommand{\tc}{\textcolor{gray}}
\newcommand{\tcr}{\textcolor{red}}
\newcommand{\tcp}{\textcolor{purple}}
\newcommand{\tco}{\textcolor{orange}}

\endinput
